$k$-Center Clustering with Outliers in the Sliding-Window Model

The $k$-center problem for a point set~$P$ asks for a collection of $k$ congruent balls (that is, balls of equal radius) that together cover all the points in $P$ and whose radius is minimized. The $k$-center problem with outliers is defined similarly, except that $z$ of the points in $P$ do need not to be covered, for a given parameter $z$. We study the $k$-center problem with outliers in data streams in the sliding-window model. In this model we are given a possibly infinite stream $P=\langle p_1,p_2,p_3,\ldots\rangle$ of points and a time window of length $W$, and we want to maintain a small sketch of the set $P(t)$ of points currently in the window such that using the sketch we can approximately solve the problem on $P(t)$. We present the first algorithm for the $k$-center problem with outliers in the sliding-window model. The algorithm works for the case where the points come from a space of bounded doubling dimension and it maintains a set $S(t)$ such that an optimal solution on $S(t)$ gives a $(1+\varepsilon)$-approximate solution on $P(t)$. The algorithm is deterministic and uses $O((kz/\varepsilon^d)\log \sigma)$ storage, where $d$ is the doubling dimension of the underlying space and $\sigma$ is the spread of the points in the stream. Algorithms providing a $(1+\varepsilon)$-approximation were not even known in the setting without outliers or in the insertion-only setting with outliers. We also present a lower bound showing that any algorithm that provides a $(1+\varepsilon)$-approximation must use $\Omega((kz/\varepsilon)\log \sigma)$ storage.

==> optiszero.tex <==
\mdb{A failed attempt to check if $\optkz(P(t))=0$.}

Before we describe our algorithm there is one technicality that we must address.
Recall that we allow the same element $x\in X$ to appear multiple times in the stream, 
so we can have $\dist(p_i,p_j)=0$ for different points in the stream. This means
that it can happen that $\optkz(P(t))=0$. To detect this, we need to maintain
some extra information. 

\begin{itemize}
\item We maintain a set $\Xrecent(t)$ that stores the $k+z+1$ elements $x\in X$ that
     have been seen most recently in $P(t)$. (If $P(t)$ contains fewer then $k+z+1$ distinct elements then $\Xrecent$ will contain fewer elements as well.)
     For each $x\in \Xrecent$ we maintain the following information.
     \begin{itemize}
         \item The number of times $x$ appeared in $P(t)$, denoted by~$n(x)$.
         \item The last time $x$ appeared, denoted by $\tlast(x)$. 
               Thus $\tlast(x) = \max \{ \at(p_i) : p_i=x \}$. \\
     \end{itemize}
\end{itemize}
Maintaining~$\Xrecent$ is done as follows. 

When a new point $p_i$ arrives we check if $p_i=x$ for some $x\in \Xrecent$.
If so, we update $\tlast(x)$ and increment $n(x)$.
If the element $p_i$ does not yet appear in $\Xrecent$ then
we add that element to $\Xrecent$ with counter~1,
\mdb{This is not correct!!}
and if we now have $|\Xrecent| > k+z+1$ then we remove the value $x$
that minimizes $\tlast(x)$ from $\Xrecent$.

When a point~$p_i$ expires \mdb{How do we know this??}
and $p_i=x$ for some $x\in \Xrecent$ we decrement $n(x)$. If we now have $n(x)=0$ , then we remove $x$
from $\Xrecent$. This is correct because no value $x'\not\in \Xrecent$
was seen after the arrival of $p_i$, so $x$ need not be replaced. 
